How to Learn and Generalize From Three Minutes of Data: Physics-Constrained and Uncertainty-Aware Neural Stochastic Differential Equations

We present a framework and algorithms to learn controlled dynamics models using neural stochastic differential equations (SDEs) -- SDEs whose drift and diffusion terms are both parametrized by neural networks. We construct the drift term to leverage a priori physics knowledge as inductive bias, and we design the diffusion term to represent a distance-aware estimate of the uncertainty in the learned model's predictions -- it matches the system's underlying stochasticity when evaluated on states near those from the training dataset, and it predicts highly stochastic dynamics when evaluated on states beyond the training regime. The proposed neural SDEs can be evaluated quickly enough for use in model predictive control algorithms, or they can be used as simulators for model-based reinforcement learning. Furthermore, they make accurate predictions over long time horizons, even when trained on small datasets that cover limited regions of the state space. We demonstrate these capabilities through experiments on simulated robotic systems, as well as by using them to model and control a hexacopter's flight dynamics: A neural SDE trained using only three minutes of manually collected flight data results in a model-based control policy that accurately tracks aggressive trajectories that push the hexacopter's velocity and Euler angles to nearly double the maximum values observed in the training dataset.

==> figures/cartpole/cartpole_rl_performance_bar_chart.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
width=0.7*\columnwidth, 
height=4.0cm,
tick align=inside,
tick pos=left,
x grid style={darkgray176},
xmin=-0.093, xmax=1.073,
xtick style={draw=none},
xticklabel style={rotate=0, font=\scriptsize},
y grid style={darkgray176},
ymin=0, ymax=644.612958758698,
ytick style={color=black},
axis y line*=left,
axis x line* = bottom,
align={center},
ylabel={\footnotesize Episodic Reward},
yticklabel style={font=\footnotesize},
xtick={0, 0.21, 0.39, 0.61, 0.80, 0.98},
xticklabels={
    \shortstack[c]{Ground Truth \\ Dynamics}, 
    \shortstack[c]{Neural SDE\\(Ours)},
    \shortstack[c]{Prob. \\ Ensemble},
    \shortstack[c]{Neural SDE \\ w/ Side Info.\\(Ours)},
    \shortstack[c]{Neural SDE\\(Ours)},
    \shortstack[c]{Prob. \\ Ensemble},
    },
ytick={0, 89, 303, 513},
yticklabels={0, 89, 303, 513},
]

\draw[draw=black, pattern=crosshatch, pattern color=groundTruth] 
(axis cs:-0.04,0) rectangle (axis cs:0.04,512.787435934102);

\draw[draw=black, pattern=crosshatch, pattern color=sdeBlackBox] 
(axis cs:0.16,0) rectangle (axis cs:0.24,508.451471328089);
\draw[draw=none, draw=black, pattern=grid, pattern color=sdeBlackBox] 
(axis cs:0.24,0) rectangle (axis cs:0.28,532.09796382886);

\draw[draw=black,pattern=crosshatch, pattern color=gaussianEnsemble] 
(axis cs:0.32,0) rectangle (axis cs:0.4,303.249820859697);
\draw[draw=black,pattern=grid, pattern color=gaussianEnsemble] 
(axis cs:0.4,0) rectangle (axis cs:0.44,320.534961018009);

\draw[draw=black,pattern=crosshatch, pattern color=sdeSideInfo] 
(axis cs:0.58,0) rectangle (axis cs:0.66,502.682927880094);
\draw[draw=black,pattern=grid, pattern color=sdeSideInfo] 
(axis cs:0.66,0) rectangle (axis cs:0.7,534.835072410437);

\draw[draw=black,pattern=crosshatch, pattern color=sdeBlackBox] 
(axis cs:0.74,0) rectangle (axis cs:0.82,447.478373237097);
\draw[draw=black,pattern=grid, pattern color=sdeBlackBox] 
(axis cs:0.82,0) rectangle (axis cs:0.86,519.798828469653);

\draw[draw=black,pattern=crosshatch, pattern color=gaussianEnsemble] 
(axis cs:0.9,0) rectangle (axis cs:0.98,88.5613818263148);
\draw[draw=black,pattern=grid, pattern color=gaussianEnsemble] 
(axis cs:0.98,0) rectangle (axis cs:1.02,581.01651229493);

\path [draw=black, semithick]
(axis cs:0,482.62239139825)
--(axis cs:0,542.952480469953);

\path [draw=black, semithick]
(axis cs:0.2,472.570529451489)
--(axis cs:0.2,544.332413204689);

\path [draw=black, semithick]
(axis cs:0.26,503.250778625692)
--(axis cs:0.26,560.945149032029);

\path [draw=black, semithick]
(axis cs:0.36,246.362454405873)
--(axis cs:0.36,360.137187313522);

\path [draw=black, semithick]
(axis cs:0.42,244.098147283769)
--(axis cs:0.42,396.971774752249);

\path [draw=black, semithick]
(axis cs:0.62,442.180654118115)
--(axis cs:0.62,563.185201642073);

\path [draw=black, semithick]
(axis cs:0.68,504.652816036883)
--(axis cs:0.68,565.01732878399);

\path [draw=black, semithick]
(axis cs:0.78,382.539134250776)
--(axis cs:0.78,512.417612223417);

\path [draw=black, semithick]
(axis cs:0.84,480.968231321273)
--(axis cs:0.84,558.629425618033);

\path [draw=black, semithick]
(axis cs:0.94,2.40959749059252)
--(axis cs:0.94,174.713166162037);

\path [draw=black, semithick]
(axis cs:1,548.115921010147)
--(axis cs:1,613.917103579712);

\addplot [semithick, black, mark=-, mark size=2, mark options={solid}, only marks]
table {%
0 482.62239139825
0.2 472.570529451489
0.26 503.250778625692
0.36 246.362454405873
0.42 244.098147283769
0.62 442.180654118115
0.68 504.652816036883
0.78 382.539134250776
0.84 480.968231321273
0.94 2.40959749059252
1 548.115921010147
};
\addplot [semithick, black, mark=-, mark size=2, mark options={solid}, only marks]
table {%
0 542.952480469953
0.2 544.332413204689
0.26 560.945149032029
0.36 360.137187313522
0.42 396.971774752249
0.62 563.185201642073
0.68 565.01732878399
0.78 512.417612223417
0.84 558.629425618033
0.94 174.713166162037
1 613.917103579712
};
\end{axis}

\draw [decorate, decoration = {calligraphic brace, mirror}, very thick] (3.9cm, 2.4cm) --  (1.7cm, 2.4cm);
\node(labelForRandomDataset) [font=\scriptsize, align=left] at (2.8cm, 2.7cm) {\shortstack[c]{\textit{random dataset}}};

\draw [decorate, decoration = {calligraphic brace, mirror}, very thick] (7.9cm, 2.4cm) --  (4.65cm, 2.4cm);
\node(labelForLearnedDataset) [font=\scriptsize, align=left] at (6.25cm, 2.7cm) {\shortstack[c]{\textit{on-policy dataset}}};

% \draw [gray, decorate, decoration = {calligraphic brace}, thick] (8.2cm, -0.1cm) --  (8.2cm, -0.9cm);
% \node(labelForLabels) [font=\scriptsize, align=left] at (9.2cm, -0.5cm) {\shortstack[l]{Model used to \\ train policy}};

\begin{customlegend}[
    legend columns=2, 
    legend style={
        align=left, 
        column sep=1.0ex, 
        font=\scriptsize, 
        % draw=white!50!black,
        draw=none,
        fill=white,
        fill opacity=0.8,
        rounded corners=1mm,
        at={(70.0mm, -10.0mm)},
    }, 
    legend entries={\shortstack[l]{Policy evaluated using \\ true dynamics}, \shortstack[l]{Policy evaluated using \\ learned dynamics}}
]
    \addlegendimage{area legend,pattern=crosshatch, pattern color=black}
    \addlegendimage{area legend,pattern=grid, pattern color=black}
\end{customlegend}

\end{tikzpicture}


==> figures/intro/sde_output_fig.tex <==
\begin{axis}[
height=3cm,
width=5cm,
axis lines=left,
tick align=inside,
tick pos=left,
xmin=-0.0, xmax=8.34749979972839,
xtick style={draw=none},
ymin=-0.317115934938192, ymax=0.268075006455183,
ytick style={draw=none},
yticklabels={''},
xticklabels={''},
axis x line shift=-0.0,
xlabel={\footnotesize Time},
xlabel style={at={(axis description cs:0.8, 0.3)}},
ylabel={\footnotesize \(\state\)},
ylabel style={rotate=-90, at={(axis description cs:0.15, 0.9)}}
]
% \path [draw=sdeBlackBox, fill=sdeBlackBox, opacity=0.1, line width=0pt]
% (axis cs:0,-0.150000005960464)
% --(axis cs:0,-0.150000005960464)
% --(axis cs:0.150000005960464,-0.213240683078766)
% --(axis cs:0.300000011920929,-0.251512259244919)
% --(axis cs:0.449999958276749,-0.252436399459839)
% --(axis cs:0.600000023841858,-0.250799983739853)
% --(axis cs:0.749999940395355,-0.264937728643417)
% --(axis cs:0.899999916553497,-0.24550798535347)
% --(axis cs:1.04999995231628,-0.250701427459717)
% --(axis cs:1.20000004768372,-0.25236913561821)
% --(axis cs:1.34999990463257,-0.290516346693039)
% --(axis cs:1.49999988079071,-0.224584132432938)
% --(axis cs:1.64999985694885,-0.201708108186722)
% --(axis cs:1.79999983310699,-0.210706532001495)
% --(axis cs:1.94999992847443,-0.199801832437515)
% --(axis cs:2.09999990463257,-0.127897784113884)
% --(axis cs:2.25,-0.0466447658836842)
% --(axis cs:2.40000009536743,-0.0547099635004997)
% --(axis cs:2.54999995231628,-0.0139910764992237)
% --(axis cs:2.69999980926514,-0.00591531535610557)
% --(axis cs:2.84999990463257,0.00127264414913952)
% --(axis cs:2.99999976158142,0.00457353424280882)
% --(axis cs:3.14999985694885,0.0112619586288929)
% --(axis cs:3.29999971389771,0.017932740971446)
% --(axis cs:3.44999980926514,0.0201629158109426)
% --(axis cs:3.59999966621399,0.0227865595370531)
% --(axis cs:3.74999976158142,0.0239233635365963)
% --(axis cs:3.89999985694885,0.0229753572493792)
% --(axis cs:4.05000019073486,0.0201440565288067)
% --(axis cs:4.19999980926514,0.0158706735819578)
% --(axis cs:4.34999990463257,0.0102954423055053)
% --(axis cs:4.5,0.00617238925769925)
% --(axis cs:4.65000009536743,0.00458752270787954)
% --(axis cs:4.80000019073486,-0.00174335308838636)
% --(axis cs:4.95000028610229,-0.00407910300418735)
% --(axis cs:5.09999990463257,-0.00909497402608395)
% --(axis cs:5.25,-0.0433969050645828)
% --(axis cs:5.39999961853027,-0.0488004200160503)
% --(axis cs:5.55000019073486,-0.118564277887344)
% --(axis cs:5.69999980926514,-0.110603265464306)
% --(axis cs:5.84999990463257,-0.127799078822136)
% --(axis cs:5.99999952316284,-0.161663308739662)
% --(axis cs:6.15000009536743,-0.188007667660713)
% --(axis cs:6.29999971389771,-0.166768461465836)
% --(axis cs:6.44999980926514,-0.149232998490334)
% --(axis cs:6.59999942779541,-0.140774682164192)
% --(axis cs:6.75,-0.128545671701431)
% --(axis cs:6.89999961853027,-0.116869412362576)
% --(axis cs:7.04999971389771,-0.0978959128260612)
% --(axis cs:7.19999933242798,-0.0808700546622276)
% --(axis cs:7.34999942779541,-0.0694963186979294)
% --(axis cs:7.49999952316284,-0.0694907605648041)
% --(axis cs:7.64999961853027,-0.0721934735774994)
% --(axis cs:7.79999971389771,-0.0664498656988144)
% --(axis cs:7.94999980926514,-0.0665964782238007)
% --(axis cs:7.94999980926514,-0.0665964782238007)
% --(axis cs:7.94999980926514,-0.0665964782238007)
% --(axis cs:7.79999971389771,-0.0664498656988144)
% --(axis cs:7.64999961853027,-0.0721934735774994)
% --(axis cs:7.49999952316284,-0.0694907605648041)
% --(axis cs:7.34999942779541,-0.0694963186979294)
% --(axis cs:7.19999933242798,-0.0808700546622276)
% --(axis cs:7.04999971389771,-0.0978959128260612)
% --(axis cs:6.89999961853027,-0.116869412362576)
% --(axis cs:6.75,-0.128545671701431)
% --(axis cs:6.59999942779541,-0.140774682164192)
% --(axis cs:6.44999980926514,-0.149232998490334)
% --(axis cs:6.29999971389771,-0.166768461465836)
% --(axis cs:6.15000009536743,-0.188007667660713)
% --(axis cs:5.99999952316284,-0.161663308739662)
% --(axis cs:5.84999990463257,-0.127799078822136)
% --(axis cs:5.69999980926514,-0.110603265464306)
% --(axis cs:5.55000019073486,-0.118564277887344)
% --(axis cs:5.39999961853027,-0.0488004200160503)
% --(axis cs:5.25,-0.0433969050645828)
% --(axis cs:5.09999990463257,-0.00909497402608395)
% --(axis cs:4.95000028610229,-0.00407910300418735)
% --(axis cs:4.80000019073486,-0.00174335308838636)
% --(axis cs:4.65000009536743,0.00458752270787954)
% --(axis cs:4.5,0.00617238925769925)
% --(axis cs:4.34999990463257,0.0102954423055053)
% --(axis cs:4.19999980926514,0.0158706735819578)
% --(axis cs:4.05000019073486,0.0201440565288067)
% --(axis cs:3.89999985694885,0.0229753572493792)
% --(axis cs:3.74999976158142,0.0239233635365963)
% --(axis cs:3.59999966621399,0.0227865595370531)
% --(axis cs:3.44999980926514,0.0201629158109426)
% --(axis cs:3.29999971389771,0.017932740971446)
% --(axis cs:3.14999985694885,0.0112619586288929)
% --(axis cs:2.99999976158142,0.00457353424280882)
% --(axis cs:2.84999990463257,0.00127264414913952)
% --(axis cs:2.69999980926514,-0.00591531535610557)
% --(axis cs:2.54999995231628,-0.0139910764992237)
% --(axis cs:2.40000009536743,-0.0547099635004997)
% --(axis cs:2.25,-0.0466447658836842)
% --(axis cs:2.09999990463257,-0.127897784113884)
% --(axis cs:1.94999992847443,-0.199801832437515)
% --(axis cs:1.79999983310699,-0.210706532001495)
% --(axis cs:1.64999985694885,-0.201708108186722)
% --(axis cs:1.49999988079071,-0.224584132432938)
% --(axis cs:1.34999990463257,-0.290516346693039)
% --(axis cs:1.20000004768372,-0.25236913561821)
% --(axis cs:1.04999995231628,-0.250701427459717)
% --(axis cs:0.899999916553497,-0.24550798535347)
% --(axis cs:0.749999940395355,-0.264937728643417)
% --(axis cs:0.600000023841858,-0.250799983739853)
% --(axis cs:0.449999958276749,-0.252436399459839)
% --(axis cs:0.300000011920929,-0.251512259244919)
% --(axis cs:0.150000005960464,-0.213240683078766)
% --(axis cs:0,-0.150000005960464)
% --cycle;

\path [draw=sdeBlackBox, fill=sdeBlackBox, opacity=0.2, line width=0pt]
(axis cs:0,-0.150000005960464)
--(axis cs:0,-0.150000005960464)
--(axis cs:0.150000005960464,-0.19937951862812)
--(axis cs:0.300000011920929,-0.231138244271278)
--(axis cs:0.449999958276749,-0.224815040826797)
--(axis cs:0.600000023841858,-0.21909262239933)
--(axis cs:0.749999940395355,-0.219632104039192)
--(axis cs:0.899999916553497,-0.211734741926193)
--(axis cs:1.04999995231628,-0.214967295527458)
--(axis cs:1.20000004768372,-0.194205433130264)
--(axis cs:1.34999990463257,-0.160251721739769)
--(axis cs:1.49999988079071,-0.173954427242279)
--(axis cs:1.64999985694885,-0.132989943027496)
--(axis cs:1.79999983310699,-0.122825056314468)
--(axis cs:1.94999992847443,-0.058933574706316)
--(axis cs:2.09999990463257,-0.0499460957944393)
--(axis cs:2.25,-0.0346952117979527)
--(axis cs:2.40000009536743,-0.0239868499338627)
--(axis cs:2.54999995231628,-0.0108405873179436)
--(axis cs:2.69999980926514,-0.000572165125049651)
--(axis cs:2.84999990463257,0.00494165346026421)
--(axis cs:2.99999976158142,0.0106086293235421)
--(axis cs:3.14999985694885,0.0182804279029369)
--(axis cs:3.29999971389771,0.0237045027315617)
--(axis cs:3.44999980926514,0.0270289946347475)
--(axis cs:3.59999966621399,0.0300558339804411)
--(axis cs:3.74999976158142,0.0308154188096523)
--(axis cs:3.89999985694885,0.029109900817275)
--(axis cs:4.05000019073486,0.0254763588309288)
--(axis cs:4.19999980926514,0.0224863141775131)
--(axis cs:4.34999990463257,0.0201820563524961)
--(axis cs:4.5,0.0152767412364483)
--(axis cs:4.65000009536743,0.00929924007505178)
--(axis cs:4.80000019073486,0.00326190609484911)
--(axis cs:4.95000028610229,-0.00338041596114635)
--(axis cs:5.09999990463257,-0.0063403001986444)
--(axis cs:5.25,-0.0111977076157928)
--(axis cs:5.39999961853027,-0.0212975852191448)
--(axis cs:5.55000019073486,-0.0293532777577639)
--(axis cs:5.69999980926514,-0.0343213751912117)
--(axis cs:5.84999990463257,-0.0354273431003094)
--(axis cs:5.99999952316284,-0.0395299419760704)
--(axis cs:6.15000009536743,-0.0397453680634499)
--(axis cs:6.29999971389771,-0.0444934107363224)
--(axis cs:6.44999980926514,-0.0463019907474518)
--(axis cs:6.59999942779541,-0.0507543347775936)
--(axis cs:6.75,-0.0493428967893124)
--(axis cs:6.89999961853027,-0.0468974523246288)
--(axis cs:7.04999971389771,-0.0497537851333618)
--(axis cs:7.19999933242798,-0.0473325103521347)
--(axis cs:7.34999942779541,-0.0443804934620857)
--(axis cs:7.49999952316284,-0.0427705682814121)
--(axis cs:7.64999961853027,-0.0343488939106464)
--(axis cs:7.79999971389771,-0.0327642634510994)
--(axis cs:7.94999980926514,-0.0307456851005554)
--(axis cs:7.94999980926514,0.0150647163391113)
--(axis cs:7.94999980926514,0.0150647163391113)
--(axis cs:7.79999971389771,0.0125132445245981)
--(axis cs:7.64999961853027,0.0127109391614795)
--(axis cs:7.49999952316284,0.0110132014378905)
--(axis cs:7.34999942779541,0.00866608507931232)
--(axis cs:7.19999933242798,0.00728022772818804)
--(axis cs:7.04999971389771,0.0070660850033164)
--(axis cs:6.89999961853027,0.00553976139053702)
--(axis cs:6.75,0.0034956440795213)
--(axis cs:6.59999942779541,0.000196917200810276)
--(axis cs:6.44999980926514,0.00284938956610858)
--(axis cs:6.29999971389771,0.00341268256306648)
--(axis cs:6.15000009536743,0.00632337480783463)
--(axis cs:5.99999952316284,0.0101506318897009)
--(axis cs:5.84999990463257,0.0115597452968359)
--(axis cs:5.69999980926514,0.0131661212071776)
--(axis cs:5.55000019073486,0.0178539175540209)
--(axis cs:5.39999961853027,0.0277676526457071)
--(axis cs:5.25,0.0442727096378803)
--(axis cs:5.09999990463257,0.0626330599188805)
--(axis cs:4.95000028610229,0.0740746408700943)
--(axis cs:4.80000019073486,0.111982621252537)
--(axis cs:4.65000009536743,0.112648919224739)
--(axis cs:4.5,0.116201609373093)
--(axis cs:4.34999990463257,0.131245464086533)
--(axis cs:4.19999980926514,0.171367600560188)
--(axis cs:4.05000019073486,0.194850653409958)
--(axis cs:3.89999985694885,0.188720881938934)
--(axis cs:3.74999976158142,0.171618923544884)
--(axis cs:3.59999966621399,0.199809119105339)
--(axis cs:3.44999980926514,0.190024822950363)
--(axis cs:3.29999971389771,0.24147541821003)
--(axis cs:3.14999985694885,0.216006711125374)
--(axis cs:2.99999976158142,0.215609818696976)
--(axis cs:2.84999990463257,0.145711600780487)
--(axis cs:2.69999980926514,0.13775822520256)
--(axis cs:2.54999995231628,0.100628174841404)
--(axis cs:2.40000009536743,0.0777141079306602)
--(axis cs:2.25,0.0405293703079224)
--(axis cs:2.09999990463257,0.0311876256018877)
--(axis cs:1.94999992847443,0.0191076435148716)
--(axis cs:1.79999983310699,-0.00904315337538719)
--(axis cs:1.64999985694885,-0.0312534533441067)
--(axis cs:1.49999988079071,-0.0533519722521305)
--(axis cs:1.34999990463257,-0.065491184592247)
--(axis cs:1.20000004768372,-0.0797302648425102)
--(axis cs:1.04999995231628,-0.0931195244193077)
--(axis cs:0.899999916553497,-0.102477207779884)
--(axis cs:0.749999940395355,-0.110583238303661)
--(axis cs:0.600000023841858,-0.106121249496937)
--(axis cs:0.449999958276749,-0.0988312736153603)
--(axis cs:0.300000011920929,-0.107206486165524)
--(axis cs:0.150000005960464,-0.111704930663109)
--(axis cs:0,-0.150000005960464)
--cycle;

% \path [draw=sdeBlackBox, fill=sdeBlackBox, opacity=0.25, line width=0pt]
% (axis cs:0,-0.150000005960464)
% --(axis cs:0,-0.150000005960464)
% --(axis cs:0.150000005960464,-0.186132863163948)
% --(axis cs:0.300000011920929,-0.213513895869255)
% --(axis cs:0.449999958276749,-0.208828061819077)
% --(axis cs:0.600000023841858,-0.196504503488541)
% --(axis cs:0.749999940395355,-0.191066578030586)
% --(axis cs:0.899999916553497,-0.194389835000038)
% --(axis cs:1.04999995231628,-0.187186062335968)
% --(axis cs:1.20000004768372,-0.169927954673767)
% --(axis cs:1.34999990463257,-0.124145813286304)
% --(axis cs:1.49999988079071,-0.101866133511066)
% --(axis cs:1.64999985694885,-0.0805356353521347)
% --(axis cs:1.79999983310699,-0.0704629272222519)
% --(axis cs:1.94999992847443,-0.0551929734647274)
% --(axis cs:2.09999990463257,-0.0446439012885094)
% --(axis cs:2.25,-0.0296341106295586)
% --(axis cs:2.40000009536743,-0.022298576310277)
% --(axis cs:2.54999995231628,-0.00427920604124665)
% --(axis cs:2.69999980926514,-0.000306511909002438)
% --(axis cs:2.84999990463257,0.00847194995731115)
% --(axis cs:2.99999976158142,0.018255427479744)
% --(axis cs:3.14999985694885,0.025410046800971)
% --(axis cs:3.29999971389771,0.0284574180841446)
% --(axis cs:3.44999980926514,0.0314994305372238)
% --(axis cs:3.59999966621399,0.0314403027296066)
% --(axis cs:3.74999976158142,0.0320304334163666)
% --(axis cs:3.89999985694885,0.0304367896169424)
% --(axis cs:4.05000019073486,0.028382133692503)
% --(axis cs:4.19999980926514,0.0255053844302893)
% --(axis cs:4.34999990463257,0.0244621820747852)
% --(axis cs:4.5,0.0168963968753815)
% --(axis cs:4.65000009536743,0.0103600453585386)
% --(axis cs:4.80000019073486,0.00678439158946276)
% --(axis cs:4.95000028610229,-0.001538653858006)
% --(axis cs:5.09999990463257,-0.00353965745307505)
% --(axis cs:5.25,-0.00713073834776878)
% --(axis cs:5.39999961853027,-0.0114728594198823)
% --(axis cs:5.55000019073486,-0.0211693309247494)
% --(axis cs:5.69999980926514,-0.0268989559262991)
% --(axis cs:5.84999990463257,-0.029477184638381)
% --(axis cs:5.99999952316284,-0.0323626212775707)
% --(axis cs:6.15000009536743,-0.0315058641135693)
% --(axis cs:6.29999971389771,-0.036984883248806)
% --(axis cs:6.44999980926514,-0.0372501276433468)
% --(axis cs:6.59999942779541,-0.038051825016737)
% --(axis cs:6.75,-0.037042822688818)
% --(axis cs:6.89999961853027,-0.0384711921215057)
% --(axis cs:7.04999971389771,-0.0386479720473289)
% --(axis cs:7.19999933242798,-0.0357139557600021)
% --(axis cs:7.34999942779541,-0.0349158458411694)
% --(axis cs:7.49999952316284,-0.0323030427098274)
% --(axis cs:7.64999961853027,-0.0335637889802456)
% --(axis cs:7.79999971389771,-0.0293243713676929)
% --(axis cs:7.94999980926514,-0.0243064612150192)
% --(axis cs:7.94999980926514,0.0109024774283171)
% --(axis cs:7.94999980926514,0.0109024774283171)
% --(axis cs:7.79999971389771,0.012338800355792)
% --(axis cs:7.64999961853027,0.00929501373320818)
% --(axis cs:7.49999952316284,0.00520857190713286)
% --(axis cs:7.34999942779541,-0.00130738283041865)
% --(axis cs:7.19999933242798,-0.00444976985454559)
% --(axis cs:7.04999971389771,-0.00551417702808976)
% --(axis cs:6.89999961853027,-0.00271120574325323)
% --(axis cs:6.75,-0.00559970270842314)
% --(axis cs:6.59999942779541,-0.00380480196326971)
% --(axis cs:6.44999980926514,-0.00145176041405648)
% --(axis cs:6.29999971389771,-0.000264371337834746)
% --(axis cs:6.15000009536743,0.00219927192665637)
% --(axis cs:5.99999952316284,0.00654659001156688)
% --(axis cs:5.84999990463257,0.00959749333560467)
% --(axis cs:5.69999980926514,0.0112298205494881)
% --(axis cs:5.55000019073486,0.0151969930157065)
% --(axis cs:5.39999961853027,0.020425371825695)
% --(axis cs:5.25,0.0253990329802036)
% --(axis cs:5.09999990463257,0.0405213870108128)
% --(axis cs:4.95000028610229,0.0667006522417068)
% --(axis cs:4.80000019073486,0.0805790424346924)
% --(axis cs:4.65000009536743,0.0886797979474068)
% --(axis cs:4.5,0.102189943194389)
% --(axis cs:4.34999990463257,0.0982924476265907)
% --(axis cs:4.19999980926514,0.105446077883244)
% --(axis cs:4.05000019073486,0.109214901924133)
% --(axis cs:3.89999985694885,0.103914462029934)
% --(axis cs:3.74999976158142,0.0859710574150085)
% --(axis cs:3.59999966621399,0.08856101334095)
% --(axis cs:3.44999980926514,0.0927065089344978)
% --(axis cs:3.29999971389771,0.0945881903171539)
% --(axis cs:3.14999985694885,0.111186139285564)
% --(axis cs:2.99999976158142,0.109735012054443)
% --(axis cs:2.84999990463257,0.108435168862343)
% --(axis cs:2.69999980926514,0.0907251387834549)
% --(axis cs:2.54999995231628,0.0601132027804852)
% --(axis cs:2.40000009536743,0.0560919232666492)
% --(axis cs:2.25,0.0348575301468372)
% --(axis cs:2.09999990463257,0.0218604914844036)
% --(axis cs:1.94999992847443,0.000482117815408856)
% --(axis cs:1.79999983310699,-0.0153585392981768)
% --(axis cs:1.64999985694885,-0.0372544936835766)
% --(axis cs:1.49999988079071,-0.0543708726763725)
% --(axis cs:1.34999990463257,-0.0709461569786072)
% --(axis cs:1.20000004768372,-0.083827406167984)
% --(axis cs:1.04999995231628,-0.0959188714623451)
% --(axis cs:0.899999916553497,-0.103202059864998)
% --(axis cs:0.749999940395355,-0.111415281891823)
% --(axis cs:0.600000023841858,-0.114783406257629)
% --(axis cs:0.449999958276749,-0.113766551017761)
% --(axis cs:0.300000011920929,-0.116837218403816)
% --(axis cs:0.150000005960464,-0.126367062330246)
% --(axis cs:0,-0.150000005960464)
% --cycle;

\path [draw=sdeBlackBox, fill=sdeBlackBox, opacity=0.3, line width=0pt]
(axis cs:0,-0.150000005960464)
--(axis cs:0,-0.150000005960464)
--(axis cs:0.150000005960464,-0.176921620965004)
--(axis cs:0.300000011920929,-0.196496456861496)
--(axis cs:0.449999958276749,-0.200725018978119)
--(axis cs:0.600000023841858,-0.193827450275421)
--(axis cs:0.749999940395355,-0.181367874145508)
--(axis cs:0.899999916553497,-0.173910245299339)
--(axis cs:1.04999995231628,-0.149890512228012)
--(axis cs:1.20000004768372,-0.136204347014427)
--(axis cs:1.34999990463257,-0.112722128629684)
--(axis cs:1.49999988079071,-0.0914430394768715)
--(axis cs:1.64999985694885,-0.0766134038567543)
--(axis cs:1.79999983310699,-0.0648159384727478)
--(axis cs:1.94999992847443,-0.0513672642409801)
--(axis cs:2.09999990463257,-0.0388887263834476)
--(axis cs:2.25,-0.0229183305054903)
--(axis cs:2.40000009536743,-0.011514063924551)
--(axis cs:2.54999995231628,0.00163060030899942)
--(axis cs:2.69999980926514,0.00728845130652189)
--(axis cs:2.84999990463257,0.0171340145170689)
--(axis cs:2.99999976158142,0.0239527300000191)
--(axis cs:3.14999985694885,0.0290216971188784)
--(axis cs:3.29999971389771,0.0325282514095306)
--(axis cs:3.44999980926514,0.0347062945365906)
--(axis cs:3.59999966621399,0.0347504541277885)
--(axis cs:3.74999976158142,0.035729356110096)
--(axis cs:3.89999985694885,0.0349140875041485)
--(axis cs:4.05000019073486,0.0343444682657719)
--(axis cs:4.19999980926514,0.0293605141341686)
--(axis cs:4.34999990463257,0.0260819923132658)
--(axis cs:4.5,0.0203887633979321)
--(axis cs:4.65000009536743,0.0154433688148856)
--(axis cs:4.80000019073486,0.0100360354408622)
--(axis cs:4.95000028610229,0.00426573073491454)
--(axis cs:5.09999990463257,0.000543521775398403)
--(axis cs:5.25,-0.00416770670562983)
--(axis cs:5.39999961853027,-0.00814981572329998)
--(axis cs:5.55000019073486,-0.0120219960808754)
--(axis cs:5.69999980926514,-0.0170698594301939)
--(axis cs:5.84999990463257,-0.0220513250678778)
--(axis cs:5.99999952316284,-0.0260059703141451)
--(axis cs:6.15000009536743,-0.0270977504551411)
--(axis cs:6.29999971389771,-0.0307329725474119)
--(axis cs:6.44999980926514,-0.0318657755851746)
--(axis cs:6.59999942779541,-0.0322539806365967)
--(axis cs:6.75,-0.0320734567940235)
--(axis cs:6.89999961853027,-0.0316953770816326)
--(axis cs:7.04999971389771,-0.0304697286337614)
--(axis cs:7.19999933242798,-0.030506731942296)
--(axis cs:7.34999942779541,-0.0291722770780325)
--(axis cs:7.49999952316284,-0.0275569763034582)
--(axis cs:7.64999961853027,-0.0260541215538979)
--(axis cs:7.79999971389771,-0.0240424908697605)
--(axis cs:7.94999980926514,-0.022404508665204)
--(axis cs:7.94999980926514,0.00494175590574741)
--(axis cs:7.94999980926514,0.00494175590574741)
--(axis cs:7.79999971389771,0.00331351649947464)
--(axis cs:7.64999961853027,0.00236241077072918)
--(axis cs:7.49999952316284,-0.00151605973951519)
--(axis cs:7.34999942779541,-0.00373104703612626)
--(axis cs:7.19999933242798,-0.00598094286397099)
--(axis cs:7.04999971389771,-0.00683369906619191)
--(axis cs:6.89999961853027,-0.00735675543546677)
--(axis cs:6.75,-0.00747158611193299)
--(axis cs:6.59999942779541,-0.00520530948415399)
--(axis cs:6.44999980926514,-0.00533252488821745)
--(axis cs:6.29999971389771,-0.00364844687283039)
--(axis cs:6.15000009536743,-0.00100709381513298)
--(axis cs:5.99999952316284,0.000363625527825207)
--(axis cs:5.84999990463257,0.00208856607787311)
--(axis cs:5.69999980926514,0.00797238759696484)
--(axis cs:5.55000019073486,0.0117653906345367)
--(axis cs:5.39999961853027,0.015142573043704)
--(axis cs:5.25,0.019270883873105)
--(axis cs:5.09999990463257,0.0256541427224874)
--(axis cs:4.95000028610229,0.0323574170470238)
--(axis cs:4.80000019073486,0.039103202521801)
--(axis cs:4.65000009536743,0.0474416837096214)
--(axis cs:4.5,0.051512822508812)
--(axis cs:4.34999990463257,0.0530836097896099)
--(axis cs:4.19999980926514,0.0573920570313931)
--(axis cs:4.05000019073486,0.0612316280603409)
--(axis cs:3.89999985694885,0.0622843727469444)
--(axis cs:3.74999976158142,0.068465568125248)
--(axis cs:3.59999966621399,0.0691353604197502)
--(axis cs:3.44999980926514,0.0727518200874329)
--(axis cs:3.29999971389771,0.0785692483186722)
--(axis cs:3.14999985694885,0.075764112174511)
--(axis cs:2.99999976158142,0.0758347436785698)
--(axis cs:2.84999990463257,0.0721858292818069)
--(axis cs:2.69999980926514,0.0654027983546257)
--(axis cs:2.54999995231628,0.052142072468996)
--(axis cs:2.40000009536743,0.0409424193203449)
--(axis cs:2.25,0.0297329761087894)
--(axis cs:2.09999990463257,0.0147562325000763)
--(axis cs:1.94999992847443,-0.00365252560004592)
--(axis cs:1.79999983310699,-0.0249834153801203)
--(axis cs:1.64999985694885,-0.0437324047088623)
--(axis cs:1.49999988079071,-0.0623137131333351)
--(axis cs:1.34999990463257,-0.076325923204422)
--(axis cs:1.20000004768372,-0.0911331325769424)
--(axis cs:1.04999995231628,-0.100815109908581)
--(axis cs:0.899999916553497,-0.105801790952682)
--(axis cs:0.749999940395355,-0.116596177220345)
--(axis cs:0.600000023841858,-0.120593972504139)
--(axis cs:0.449999958276749,-0.126609668135643)
--(axis cs:0.300000011920929,-0.127182900905609)
--(axis cs:0.150000005960464,-0.136518716812134)
--(axis cs:0,-0.150000005960464)
--cycle;

% \path [draw=sdeBlackBox, fill=sdeBlackBox, opacity=0.35, line width=0pt]
% (axis cs:0,-0.150000005960464)
% --(axis cs:0,-0.150000005960464)
% --(axis cs:0.150000005960464,-0.174554005265236)
% --(axis cs:0.300000011920929,-0.192253142595291)
% --(axis cs:0.449999958276749,-0.19048860669136)
% --(axis cs:0.600000023841858,-0.181367114186287)
% --(axis cs:0.749999940395355,-0.16818730533123)
% --(axis cs:0.899999916553497,-0.160179287195206)
% --(axis cs:1.04999995231628,-0.142764568328857)
% --(axis cs:1.20000004768372,-0.124087236821651)
% --(axis cs:1.34999990463257,-0.108990877866745)
% --(axis cs:1.49999988079071,-0.0886800214648247)
% --(axis cs:1.64999985694885,-0.0724661573767662)
% --(axis cs:1.79999983310699,-0.0593817010521889)
% --(axis cs:1.94999992847443,-0.0464465022087097)
% --(axis cs:2.09999990463257,-0.0319566465914249)
% --(axis cs:2.25,-0.0210251547396183)
% --(axis cs:2.40000009536743,-0.00777550507336855)
% --(axis cs:2.54999995231628,0.00573972566053271)
% --(axis cs:2.69999980926514,0.0119103053584695)
% --(axis cs:2.84999990463257,0.0235282946377993)
% --(axis cs:2.99999976158142,0.0313326120376587)
% --(axis cs:3.14999985694885,0.033126562833786)
% --(axis cs:3.29999971389771,0.0372971743345261)
% --(axis cs:3.44999980926514,0.0405699051916599)
% --(axis cs:3.59999966621399,0.0371407940983772)
% --(axis cs:3.74999976158142,0.0411007218062878)
% --(axis cs:3.89999985694885,0.0391494520008564)
% --(axis cs:4.05000019073486,0.0355840884149075)
% --(axis cs:4.19999980926514,0.03309665620327)
% --(axis cs:4.34999990463257,0.0279124807566404)
% --(axis cs:4.5,0.0225250646471977)
% --(axis cs:4.65000009536743,0.0166964251548052)
% --(axis cs:4.80000019073486,0.0116619365289807)
% --(axis cs:4.95000028610229,0.00663224188610911)
% --(axis cs:5.09999990463257,0.0022216783836484)
% --(axis cs:5.25,-0.00243206741288304)
% --(axis cs:5.39999961853027,-0.00732679571956396)
% --(axis cs:5.55000019073486,-0.0116421459242702)
% --(axis cs:5.69999980926514,-0.0157999154180288)
% --(axis cs:5.84999990463257,-0.0191462878137827)
% --(axis cs:5.99999952316284,-0.0222486723214388)
% --(axis cs:6.15000009536743,-0.0243207421153784)
% --(axis cs:6.29999971389771,-0.0276079569011927)
% --(axis cs:6.44999980926514,-0.0290860887616873)
% --(axis cs:6.59999942779541,-0.0310017559677362)
% --(axis cs:6.75,-0.0306203700602055)
% --(axis cs:6.89999961853027,-0.0308659803122282)
% --(axis cs:7.04999971389771,-0.0288535635918379)
% --(axis cs:7.19999933242798,-0.0286649130284786)
% --(axis cs:7.34999942779541,-0.0265866238623857)
% --(axis cs:7.49999952316284,-0.0260945484042168)
% --(axis cs:7.64999961853027,-0.0256354603916407)
% --(axis cs:7.79999971389771,-0.0223955903202295)
% --(axis cs:7.94999980926514,-0.0200993437319994)
% --(axis cs:7.94999980926514,0.000501677219290286)
% --(axis cs:7.94999980926514,0.000501677219290286)
% --(axis cs:7.79999971389771,-0.0027061605360359)
% --(axis cs:7.64999961853027,-0.00510346610099077)
% --(axis cs:7.49999952316284,-0.00492360210046172)
% --(axis cs:7.34999942779541,-0.00628288183361292)
% --(axis cs:7.19999933242798,-0.00767234666272998)
% --(axis cs:7.04999971389771,-0.00962112564593554)
% --(axis cs:6.89999961853027,-0.00996705610305071)
% --(axis cs:6.75,-0.00865283515304327)
% --(axis cs:6.59999942779541,-0.00815032236278057)
% --(axis cs:6.44999980926514,-0.00797715969383717)
% --(axis cs:6.29999971389771,-0.00613643508404493)
% --(axis cs:6.15000009536743,-0.00541451387107372)
% --(axis cs:5.99999952316284,-0.00435069901868701)
% --(axis cs:5.84999990463257,-0.00101944350171834)
% --(axis cs:5.69999980926514,0.00257972907274961)
% --(axis cs:5.55000019073486,0.00628624577075243)
% --(axis cs:5.39999961853027,0.0122681278735399)
% --(axis cs:5.25,0.01751952432096)
% --(axis cs:5.09999990463257,0.0230093095451593)
% --(axis cs:4.95000028610229,0.0268475990742445)
% --(axis cs:4.80000019073486,0.0318937785923481)
% --(axis cs:4.65000009536743,0.0394759029150009)
% --(axis cs:4.5,0.043567705899477)
% --(axis cs:4.34999990463257,0.0493790470063686)
% --(axis cs:4.19999980926514,0.0541156195104122)
% --(axis cs:4.05000019073486,0.0556228794157505)
% --(axis cs:3.89999985694885,0.0601222924888134)
% --(axis cs:3.74999976158142,0.0636626183986664)
% --(axis cs:3.59999966621399,0.0662743002176285)
% --(axis cs:3.44999980926514,0.0672198385000229)
% --(axis cs:3.29999971389771,0.0693742334842682)
% --(axis cs:3.14999985694885,0.0715922340750694)
% --(axis cs:2.99999976158142,0.0650506913661957)
% --(axis cs:2.84999990463257,0.0678382366895676)
% --(axis cs:2.69999980926514,0.056366391479969)
% --(axis cs:2.54999995231628,0.0437346622347832)
% --(axis cs:2.40000009536743,0.0367615558207035)
% --(axis cs:2.25,0.0223016701638699)
% --(axis cs:2.09999990463257,0.00818460900336504)
% --(axis cs:1.94999992847443,-0.0102943060919642)
% --(axis cs:1.79999983310699,-0.0312374141067266)
% --(axis cs:1.64999985694885,-0.0460265800356865)
% --(axis cs:1.49999988079071,-0.0630528405308723)
% --(axis cs:1.34999990463257,-0.080931656062603)
% --(axis cs:1.20000004768372,-0.0930581912398338)
% --(axis cs:1.04999995231628,-0.103133112192154)
% --(axis cs:0.899999916553497,-0.114011369645596)
% --(axis cs:0.749999940395355,-0.121141776442528)
% --(axis cs:0.600000023841858,-0.126737788319588)
% --(axis cs:0.449999958276749,-0.136757910251617)
% --(axis cs:0.300000011920929,-0.138379201292992)
% --(axis cs:0.150000005960464,-0.140209779143333)
% --(axis cs:0,-0.150000005960464)
% --cycle;

\path [draw=sdeBlackBox, fill=sdeBlackBox, opacity=0.4, line width=0pt]
(axis cs:0,-0.150000005960464)
--(axis cs:0,-0.150000005960464)
--(axis cs:0.150000005960464,-0.173972487449646)
--(axis cs:0.300000011920929,-0.18795582652092)
--(axis cs:0.449999958276749,-0.180714890360832)
--(axis cs:0.600000023841858,-0.169900566339493)
--(axis cs:0.749999940395355,-0.160584926605225)
--(axis cs:0.899999916553497,-0.149133518338203)
--(axis cs:1.04999995231628,-0.140928819775581)
--(axis cs:1.20000004768372,-0.120857007801533)
--(axis cs:1.34999990463257,-0.10539898276329)
--(axis cs:1.49999988079071,-0.0861813724040985)
--(axis cs:1.64999985694885,-0.0704793632030487)
--(axis cs:1.79999983310699,-0.0578248836100101)
--(axis cs:1.94999992847443,-0.0454141311347485)
--(axis cs:2.09999990463257,-0.0296723116189241)
--(axis cs:2.25,-0.0178919658064842)
--(axis cs:2.40000009536743,-0.00386401498690248)
--(axis cs:2.54999995231628,0.00709430919960141)
--(axis cs:2.69999980926514,0.0186363980174065)
--(axis cs:2.84999990463257,0.0271824114024639)
--(axis cs:2.99999976158142,0.0336373224854469)
--(axis cs:3.14999985694885,0.0379294194281101)
--(axis cs:3.29999971389771,0.0394054874777794)
--(axis cs:3.44999980926514,0.0419401787221432)
--(axis cs:3.59999966621399,0.0425657145678997)
--(axis cs:3.74999976158142,0.041782058775425)
--(axis cs:3.89999985694885,0.0402654409408569)
--(axis cs:4.05000019073486,0.038200993090868)
--(axis cs:4.19999980926514,0.0350703969597816)
--(axis cs:4.34999990463257,0.0284291189163923)
--(axis cs:4.5,0.0243818666785955)
--(axis cs:4.65000009536743,0.0185990799218416)
--(axis cs:4.80000019073486,0.0130385356023908)
--(axis cs:4.95000028610229,0.00813212711364031)
--(axis cs:5.09999990463257,0.00480390712618828)
--(axis cs:5.25,-0.00158089806791395)
--(axis cs:5.39999961853027,-0.00610357569530606)
--(axis cs:5.55000019073486,-0.0103119136765599)
--(axis cs:5.69999980926514,-0.014475486241281)
--(axis cs:5.84999990463257,-0.0180019214749336)
--(axis cs:5.99999952316284,-0.0214822255074978)
--(axis cs:6.15000009536743,-0.0235321074724197)
--(axis cs:6.29999971389771,-0.026590570807457)
--(axis cs:6.44999980926514,-0.028464712202549)
--(axis cs:6.59999942779541,-0.0306391809135675)
--(axis cs:6.75,-0.0289781838655472)
--(axis cs:6.89999961853027,-0.0299434568732977)
--(axis cs:7.04999971389771,-0.0281276982277632)
--(axis cs:7.19999933242798,-0.0271146986633539)
--(axis cs:7.34999942779541,-0.0258832406252623)
--(axis cs:7.49999952316284,-0.0256583392620087)
--(axis cs:7.64999961853027,-0.0240549482405186)
--(axis cs:7.79999971389771,-0.0210155453532934)
--(axis cs:7.94999980926514,-0.0197816342115402)
--(axis cs:7.94999980926514,-0.00286366161890328)
--(axis cs:7.94999980926514,-0.00286366161890328)
--(axis cs:7.79999971389771,-0.00433320458978415)
--(axis cs:7.64999961853027,-0.00612888159230351)
--(axis cs:7.49999952316284,-0.00621885806322098)
--(axis cs:7.34999942779541,-0.00753017887473106)
--(axis cs:7.19999933242798,-0.00958677567541599)
--(axis cs:7.04999971389771,-0.0105567229911685)
--(axis cs:6.89999961853027,-0.0108129614964128)
--(axis cs:6.75,-0.0111685646697879)
--(axis cs:6.59999942779541,-0.0101572833955288)
--(axis cs:6.44999980926514,-0.00836005434393883)
--(axis cs:6.29999971389771,-0.00732652749866247)
--(axis cs:6.15000009536743,-0.00687604723498225)
--(axis cs:5.99999952316284,-0.00567881856113672)
--(axis cs:5.84999990463257,-0.0046174731105566)
--(axis cs:5.69999980926514,0.00152774143498391)
--(axis cs:5.55000019073486,0.00460956757888198)
--(axis cs:5.39999961853027,0.0118075208738446)
--(axis cs:5.25,0.0168502442538738)
--(axis cs:5.09999990463257,0.0215311590582132)
--(axis cs:4.95000028610229,0.0262846946716309)
--(axis cs:4.80000019073486,0.0309234205633402)
--(axis cs:4.65000009536743,0.0373704098165035)
--(axis cs:4.5,0.0429720282554626)
--(axis cs:4.34999990463257,0.0477412305772305)
--(axis cs:4.19999980926514,0.0498626604676247)
--(axis cs:4.05000019073486,0.0548252612352371)
--(axis cs:3.89999985694885,0.0588054321706295)
--(axis cs:3.74999976158142,0.0633158534765244)
--(axis cs:3.59999966621399,0.0646934732794762)
--(axis cs:3.44999980926514,0.0667062178254128)
--(axis cs:3.29999971389771,0.066399447619915)
--(axis cs:3.14999985694885,0.0665472894906998)
--(axis cs:2.99999976158142,0.0612504743039608)
--(axis cs:2.84999990463257,0.0589702539145947)
--(axis cs:2.69999980926514,0.0517183616757393)
--(axis cs:2.54999995231628,0.0428683422505856)
--(axis cs:2.40000009536743,0.033403430134058)
--(axis cs:2.25,0.0187537539750338)
--(axis cs:2.09999990463257,0.0020039186347276)
--(axis cs:1.94999992847443,-0.0113453110679984)
--(axis cs:1.79999983310699,-0.033075712621212)
--(axis cs:1.64999985694885,-0.0498392730951309)
--(axis cs:1.49999988079071,-0.0660983175039291)
--(axis cs:1.34999990463257,-0.0818383619189262)
--(axis cs:1.20000004768372,-0.0938942581415176)
--(axis cs:1.04999995231628,-0.104559980332851)
--(axis cs:0.899999916553497,-0.118171751499176)
--(axis cs:0.749999940395355,-0.122653432190418)
--(axis cs:0.600000023841858,-0.13235267996788)
--(axis cs:0.449999958276749,-0.139166131615639)
--(axis cs:0.300000011920929,-0.141142562031746)
--(axis cs:0.150000005960464,-0.142805308103561)
--(axis cs:0,-0.150000005960464)
--cycle;

% \path [draw=sdeBlackBox, fill=sdeBlackBox, opacity=0.45, line width=0pt]
% (axis cs:0,-0.150000005960464)
% --(axis cs:0,-0.150000005960464)
% --(axis cs:0.150000005960464,-0.172352612018585)
% --(axis cs:0.300000011920929,-0.179145693778992)
% --(axis cs:0.449999958276749,-0.164947092533112)
% --(axis cs:0.600000023841858,-0.167206451296806)
% --(axis cs:0.749999940395355,-0.157365515828133)
% --(axis cs:0.899999916553497,-0.147011175751686)
% --(axis cs:1.04999995231628,-0.13327656686306)
% --(axis cs:1.20000004768372,-0.11784503608942)
% --(axis cs:1.34999990463257,-0.100937515497208)
% --(axis cs:1.49999988079071,-0.0835612118244171)
% --(axis cs:1.64999985694885,-0.0681304037570953)
% --(axis cs:1.79999983310699,-0.0562689788639545)
% --(axis cs:1.94999992847443,-0.0425137244164944)
% --(axis cs:2.09999990463257,-0.0289473067969084)
% --(axis cs:2.25,-0.0131205078214407)
% --(axis cs:2.40000009536743,-0.00018542556790635)
% --(axis cs:2.54999995231628,0.0112212626263499)
% --(axis cs:2.69999980926514,0.0207897648215294)
% --(axis cs:2.84999990463257,0.0284139364957809)
% --(axis cs:2.99999976158142,0.0365373902022839)
% --(axis cs:3.14999985694885,0.0393433645367622)
% --(axis cs:3.29999971389771,0.0432558879256248)
% --(axis cs:3.44999980926514,0.0452673733234406)
% --(axis cs:3.59999966621399,0.0441600009799004)
% --(axis cs:3.74999976158142,0.0431052036583424)
% --(axis cs:3.89999985694885,0.0438815541565418)
% --(axis cs:4.05000019073486,0.0415718480944633)
% --(axis cs:4.19999980926514,0.0368839763104916)
% --(axis cs:4.34999990463257,0.0326732024550438)
% --(axis cs:4.5,0.0271815620362759)
% --(axis cs:4.65000009536743,0.0219876524060965)
% --(axis cs:4.80000019073486,0.016552746295929)
% --(axis cs:4.95000028610229,0.011491859331727)
% --(axis cs:5.09999990463257,0.00578415300697088)
% --(axis cs:5.25,-0.000246063806116581)
% --(axis cs:5.39999961853027,-0.00485625909641385)
% --(axis cs:5.55000019073486,-0.00871587265282869)
% --(axis cs:5.69999980926514,-0.0120760500431061)
% --(axis cs:5.84999990463257,-0.0161499865353107)
% --(axis cs:5.99999952316284,-0.0192608125507832)
% --(axis cs:6.15000009536743,-0.0213967375457287)
% --(axis cs:6.29999971389771,-0.024724218994379)
% --(axis cs:6.44999980926514,-0.0271835550665855)
% --(axis cs:6.59999942779541,-0.0284886602312326)
% --(axis cs:6.75,-0.0268225688487291)
% --(axis cs:6.89999961853027,-0.0263301096856594)
% --(axis cs:7.04999971389771,-0.0261102896183729)
% --(axis cs:7.19999933242798,-0.0254785120487213)
% --(axis cs:7.34999942779541,-0.0252372343093157)
% --(axis cs:7.49999952316284,-0.0238334927707911)
% --(axis cs:7.64999961853027,-0.022878160700202)
% --(axis cs:7.79999971389771,-0.019688980653882)
% --(axis cs:7.94999980926514,-0.0177097916603088)
% --(axis cs:7.94999980926514,-0.00447673723101616)
% --(axis cs:7.94999980926514,-0.00447673723101616)
% --(axis cs:7.79999971389771,-0.00614250358194113)
% --(axis cs:7.64999961853027,-0.00660716602578759)
% --(axis cs:7.49999952316284,-0.00839997176080942)
% --(axis cs:7.34999942779541,-0.00899599865078926)
% --(axis cs:7.19999933242798,-0.0107582425698638)
% --(axis cs:7.04999971389771,-0.0113300895318389)
% --(axis cs:6.89999961853027,-0.012802867218852)
% --(axis cs:6.75,-0.0121339950710535)
% --(axis cs:6.59999942779541,-0.0118967099115252)
% --(axis cs:6.44999980926514,-0.0127514265477657)
% --(axis cs:6.29999971389771,-0.0105030005797744)
% --(axis cs:6.15000009536743,-0.0101893842220306)
% --(axis cs:5.99999952316284,-0.00857826601713896)
% --(axis cs:5.84999990463257,-0.00552076892927289)
% --(axis cs:5.69999980926514,-0.00037013998371549)
% --(axis cs:5.55000019073486,0.00338273961097002)
% --(axis cs:5.39999961853027,0.00881868228316307)
% --(axis cs:5.25,0.0135936085134745)
% --(axis cs:5.09999990463257,0.0188281126320362)
% --(axis cs:4.95000028610229,0.0247788317501545)
% --(axis cs:4.80000019073486,0.0300093833357096)
% --(axis cs:4.65000009536743,0.0353790335357189)
% --(axis cs:4.5,0.0410574153065681)
% --(axis cs:4.34999990463257,0.0456852726638317)
% --(axis cs:4.19999980926514,0.0494475401937962)
% --(axis cs:4.05000019073486,0.0530068799853325)
% --(axis cs:3.89999985694885,0.0554383657872677)
% --(axis cs:3.74999976158142,0.0583878569304943)
% --(axis cs:3.59999966621399,0.0634874477982521)
% --(axis cs:3.44999980926514,0.0637282207608223)
% --(axis cs:3.29999971389771,0.0645047575235367)
% --(axis cs:3.14999985694885,0.0619026273488998)
% --(axis cs:2.99999976158142,0.0592251643538475)
% --(axis cs:2.84999990463257,0.051328282803297)
% --(axis cs:2.69999980926514,0.0457722321152687)
% --(axis cs:2.54999995231628,0.0386009737849236)
% --(axis cs:2.40000009536743,0.0264329332858324)
% --(axis cs:2.25,0.00470671057701111)
% --(axis cs:2.09999990463257,-0.0080257086083293)
% --(axis cs:1.94999992847443,-0.0189025849103928)
% --(axis cs:1.79999983310699,-0.0371660776436329)
% --(axis cs:1.64999985694885,-0.0547306425869465)
% --(axis cs:1.49999988079071,-0.0689181163907051)
% --(axis cs:1.34999990463257,-0.0827730968594551)
% --(axis cs:1.20000004768372,-0.0952193886041641)
% --(axis cs:1.04999995231628,-0.106769643723965)
% --(axis cs:0.899999916553497,-0.120496436953545)
% --(axis cs:0.749999940395355,-0.125783383846283)
% --(axis cs:0.600000023841858,-0.134638205170631)
% --(axis cs:0.449999958276749,-0.142671927809715)
% --(axis cs:0.300000011920929,-0.143981769680977)
% --(axis cs:0.150000005960464,-0.145146638154984)
% --(axis cs:0,-0.150000005960464)
% --cycle;

\path [draw=sdeBlackBox, fill=sdeBlackBox, opacity=0.5, line width=0pt]
(axis cs:0,-0.150000005960464)
--(axis cs:0,-0.150000005960464)
--(axis cs:0.150000005960464,-0.170996442437172)
--(axis cs:0.300000011920929,-0.170309528708458)
--(axis cs:0.449999958276749,-0.161423817276955)
--(axis cs:0.600000023841858,-0.166006326675415)
--(axis cs:0.749999940395355,-0.153737679123878)
--(axis cs:0.899999916553497,-0.142585203051567)
--(axis cs:1.04999995231628,-0.130439236760139)
--(axis cs:1.20000004768372,-0.117153741419315)
--(axis cs:1.34999990463257,-0.0995783060789108)
--(axis cs:1.49999988079071,-0.0828055664896965)
--(axis cs:1.64999985694885,-0.0667144134640694)
--(axis cs:1.79999983310699,-0.0544039979577065)
--(axis cs:1.94999992847443,-0.0413874574005604)
--(axis cs:2.09999990463257,-0.0260065868496895)
--(axis cs:2.25,-0.0101357456296682)
--(axis cs:2.40000009536743,0.00190396094694734)
--(axis cs:2.54999995231628,0.0134037816897035)
--(axis cs:2.69999980926514,0.0214715860784054)
--(axis cs:2.84999990463257,0.0307690408080816)
--(axis cs:2.99999976158142,0.0381216816604137)
--(axis cs:3.14999985694885,0.0417731143534184)
--(axis cs:3.29999971389771,0.0440880805253983)
--(axis cs:3.44999980926514,0.045646820217371)
--(axis cs:3.59999966621399,0.0448261871933937)
--(axis cs:3.74999976158142,0.0442836284637451)
--(axis cs:3.89999985694885,0.0441564545035362)
--(axis cs:4.05000019073486,0.0427125580608845)
--(axis cs:4.19999980926514,0.037575826048851)
--(axis cs:4.34999990463257,0.0335823558270931)
--(axis cs:4.5,0.0274091940373182)
--(axis cs:4.65000009536743,0.0244663264602423)
--(axis cs:4.80000019073486,0.0173277780413628)
--(axis cs:4.95000028610229,0.0130330007523298)
--(axis cs:5.09999990463257,0.00725461263209581)
--(axis cs:5.25,0.000341624749125913)
--(axis cs:5.39999961853027,-0.0044399774633348)
--(axis cs:5.55000019073486,-0.00731984060257673)
--(axis cs:5.69999980926514,-0.0114495195448399)
--(axis cs:5.84999990463257,-0.0154647277668118)
--(axis cs:5.99999952316284,-0.0183444656431675)
--(axis cs:6.15000009536743,-0.020871514454484)
--(axis cs:6.29999971389771,-0.0228825770318508)
--(axis cs:6.44999980926514,-0.0264857299625874)
--(axis cs:6.59999942779541,-0.0283157639205456)
--(axis cs:6.75,-0.0264779813587666)
--(axis cs:6.89999961853027,-0.0251788776367903)
--(axis cs:7.04999971389771,-0.0243105702102184)
--(axis cs:7.19999933242798,-0.0245121940970421)
--(axis cs:7.34999942779541,-0.0235051400959492)
--(axis cs:7.49999952316284,-0.0225233472883701)
--(axis cs:7.64999961853027,-0.0216934699565172)
--(axis cs:7.79999971389771,-0.018793523311615)
--(axis cs:7.94999980926514,-0.0174104906618595)
--(axis cs:7.94999980926514,-0.0062820166349411)
--(axis cs:7.94999980926514,-0.0062820166349411)
--(axis cs:7.79999971389771,-0.00624022167176008)
--(axis cs:7.64999961853027,-0.00770709058269858)
--(axis cs:7.49999952316284,-0.010357272811234)
--(axis cs:7.34999942779541,-0.00962329842150211)
--(axis cs:7.19999933242798,-0.0116085214540362)
--(axis cs:7.04999971389771,-0.0128566166386008)
--(axis cs:6.89999961853027,-0.0134903816506267)
--(axis cs:6.75,-0.0126002328470349)
--(axis cs:6.59999942779541,-0.0127354245632887)
--(axis cs:6.44999980926514,-0.0134429596364498)
--(axis cs:6.29999971389771,-0.0123835606500506)
--(axis cs:6.15000009536743,-0.0117605412378907)
--(axis cs:5.99999952316284,-0.00920414458960295)
--(axis cs:5.84999990463257,-0.00705564301460981)
--(axis cs:5.69999980926514,-0.003003871999681)
--(axis cs:5.55000019073486,0.00214859494008124)
--(axis cs:5.39999961853027,0.00738651258870959)
--(axis cs:5.25,0.0111163388937712)
--(axis cs:5.09999990463257,0.0178810674697161)
--(axis cs:4.95000028610229,0.0244811940938234)
--(axis cs:4.80000019073486,0.0286896638572216)
--(axis cs:4.65000009536743,0.0340320505201817)
--(axis cs:4.5,0.0391814820468426)
--(axis cs:4.34999990463257,0.0429122745990753)
--(axis cs:4.19999980926514,0.0471580065786839)
--(axis cs:4.05000019073486,0.0512384511530399)
--(axis cs:3.89999985694885,0.053133137524128)
--(axis cs:3.74999976158142,0.0580593310296535)
--(axis cs:3.59999966621399,0.0614144131541252)
--(axis cs:3.44999980926514,0.0629881918430328)
--(axis cs:3.29999971389771,0.0622753724455833)
--(axis cs:3.14999985694885,0.0601550415158272)
--(axis cs:2.99999976158142,0.0564239025115967)
--(axis cs:2.84999990463257,0.0502088516950607)
--(axis cs:2.69999980926514,0.0431001409888268)
--(axis cs:2.54999995231628,0.0327219069004059)
--(axis cs:2.40000009536743,0.0158421527594328)
--(axis cs:2.25,0.00343925203196704)
--(axis cs:2.09999990463257,-0.00955395959317684)
--(axis cs:1.94999992847443,-0.0248807892203331)
--(axis cs:1.79999983310699,-0.0398938208818436)
--(axis cs:1.64999985694885,-0.0550093576312065)
--(axis cs:1.49999988079071,-0.0716889277100563)
--(axis cs:1.34999990463257,-0.0836176201701164)
--(axis cs:1.20000004768372,-0.0992400124669075)
--(axis cs:1.04999995231628,-0.110049359500408)
--(axis cs:0.899999916553497,-0.123696222901344)
--(axis cs:0.749999940395355,-0.127207145094872)
--(axis cs:0.600000023841858,-0.137323692440987)
--(axis cs:0.449999958276749,-0.143685966730118)
--(axis cs:0.300000011920929,-0.145355194807053)
--(axis cs:0.150000005960464,-0.14957357943058)
--(axis cs:0,-0.150000005960464)
--cycle;

% \path [draw=sdeBlackBox, fill=sdeBlackBox, opacity=0.55, line width=0pt]
% (axis cs:0,-0.150000005960464)
% --(axis cs:0,-0.150000005960464)
% --(axis cs:0.150000005960464,-0.16526597738266)
% --(axis cs:0.300000011920929,-0.164174512028694)
% --(axis cs:0.449999958276749,-0.159713178873062)
% --(axis cs:0.600000023841858,-0.159402593970299)
% --(axis cs:0.749999940395355,-0.147760465741158)
% --(axis cs:0.899999916553497,-0.140307545661926)
% --(axis cs:1.04999995231628,-0.128587052226067)
% --(axis cs:1.20000004768372,-0.11231405287981)
% --(axis cs:1.34999990463257,-0.0979153737425804)
% --(axis cs:1.49999988079071,-0.0812643244862556)
% --(axis cs:1.64999985694885,-0.0658998712897301)
% --(axis cs:1.79999983310699,-0.0520634911954403)
% --(axis cs:1.94999992847443,-0.0361107513308525)
% --(axis cs:2.09999990463257,-0.0213032867759466)
% --(axis cs:2.25,-0.00788893643766642)
% --(axis cs:2.40000009536743,0.00467482162639499)
% --(axis cs:2.54999995231628,0.0182155575603247)
% --(axis cs:2.69999980926514,0.0251785088330507)
% --(axis cs:2.84999990463257,0.0317287184298038)
% --(axis cs:2.99999976158142,0.0385332070291042)
% --(axis cs:3.14999985694885,0.0431074574589729)
% --(axis cs:3.29999971389771,0.0462564677000046)
% --(axis cs:3.44999980926514,0.0475030951201916)
% --(axis cs:3.59999966621399,0.0483561903238297)
% --(axis cs:3.74999976158142,0.0477461814880371)
% --(axis cs:3.89999985694885,0.046283271163702)
% --(axis cs:4.05000019073486,0.0429003164172173)
% --(axis cs:4.19999980926514,0.0396032743155956)
% --(axis cs:4.34999990463257,0.0353392474353313)
% --(axis cs:4.5,0.0289835184812546)
% --(axis cs:4.65000009536743,0.0254858937114477)
% --(axis cs:4.80000019073486,0.019206166267395)
% --(axis cs:4.95000028610229,0.0135015156120062)
% --(axis cs:5.09999990463257,0.00799399148672819)
% --(axis cs:5.25,0.00273504620417953)
% --(axis cs:5.39999961853027,-0.00205324240960181)
% --(axis cs:5.55000019073486,-0.00648711901158094)
% --(axis cs:5.69999980926514,-0.0102573381736875)
% --(axis cs:5.84999990463257,-0.0132349552586675)
% --(axis cs:5.99999952316284,-0.0172490477561951)
% --(axis cs:6.15000009536743,-0.0202724635601044)
% --(axis cs:6.29999971389771,-0.020975437015295)
% --(axis cs:6.44999980926514,-0.0251733940094709)
% --(axis cs:6.59999942779541,-0.0251523815095425)
% --(axis cs:6.75,-0.0237297490239143)
% --(axis cs:6.89999961853027,-0.0227625425904989)
% --(axis cs:7.04999971389771,-0.0218143817037344)
% --(axis cs:7.19999933242798,-0.0206871647387743)
% --(axis cs:7.34999942779541,-0.019646167755127)
% --(axis cs:7.49999952316284,-0.0194352213293314)
% --(axis cs:7.64999961853027,-0.0191022865474224)
% --(axis cs:7.79999971389771,-0.0174523089081049)
% --(axis cs:7.94999980926514,-0.0164800230413675)
% --(axis cs:7.94999980926514,-0.00704689277336001)
% --(axis cs:7.94999980926514,-0.00704689277336001)
% --(axis cs:7.79999971389771,-0.00757340062409639)
% --(axis cs:7.64999961853027,-0.00954926479607821)
% --(axis cs:7.49999952316284,-0.0112118059769273)
% --(axis cs:7.34999942779541,-0.0128436498343945)
% --(axis cs:7.19999933242798,-0.0123578887432814)
% --(axis cs:7.04999971389771,-0.0135898785665631)
% --(axis cs:6.89999961853027,-0.014361884444952)
% --(axis cs:6.75,-0.0150642059743404)
% --(axis cs:6.59999942779541,-0.0132474452257156)
% --(axis cs:6.44999980926514,-0.0143162189051509)
% --(axis cs:6.29999971389771,-0.015814671292901)
% --(axis cs:6.15000009536743,-0.012815679423511)
% --(axis cs:5.99999952316284,-0.0120181869715452)
% --(axis cs:5.84999990463257,-0.0083503145724535)
% --(axis cs:5.69999980926514,-0.00469935964792967)
% --(axis cs:5.55000019073486,0.00090688606724143)
% --(axis cs:5.39999961853027,0.00545796332880855)
% --(axis cs:5.25,0.00943976454436779)
% --(axis cs:5.09999990463257,0.0148626714944839)
% --(axis cs:4.95000028610229,0.0212576072663069)
% --(axis cs:4.80000019073486,0.0264247730374336)
% --(axis cs:4.65000009536743,0.0324666425585747)
% --(axis cs:4.5,0.0359704867005348)
% --(axis cs:4.34999990463257,0.0384125933051109)
% --(axis cs:4.19999980926514,0.0446003302931786)
% --(axis cs:4.05000019073486,0.048665814101696)
% --(axis cs:3.89999985694885,0.0510674603283405)
% --(axis cs:3.74999976158142,0.0564040690660477)
% --(axis cs:3.59999966621399,0.056672029197216)
% --(axis cs:3.44999980926514,0.059312030673027)
% --(axis cs:3.29999971389771,0.0590704530477524)
% --(axis cs:3.14999985694885,0.0576660856604576)
% --(axis cs:2.99999976158142,0.052711233496666)
% --(axis cs:2.84999990463257,0.0437945052981377)
% --(axis cs:2.69999980926514,0.0371026769280434)
% --(axis cs:2.54999995231628,0.0281304456293583)
% --(axis cs:2.40000009536743,0.0138751892372966)
% --(axis cs:2.25,0.00229458068497479)
% --(axis cs:2.09999990463257,-0.0124347656965256)
% --(axis cs:1.94999992847443,-0.0267866030335426)
% --(axis cs:1.79999983310699,-0.0427738763391972)
% --(axis cs:1.64999985694885,-0.0617663897573948)
% --(axis cs:1.49999988079071,-0.0723584368824959)
% --(axis cs:1.34999990463257,-0.0862068086862564)
% --(axis cs:1.20000004768372,-0.0999302268028259)
% --(axis cs:1.04999995231628,-0.112983919680119)
% --(axis cs:0.899999916553497,-0.12429565936327)
% --(axis cs:0.749999940395355,-0.13310731947422)
% --(axis cs:0.600000023841858,-0.140864953398705)
% --(axis cs:0.449999958276749,-0.147948950529099)
% --(axis cs:0.300000011920929,-0.155076697468758)
% --(axis cs:0.150000005960464,-0.155474036931992)
% --(axis cs:0,-0.150000005960464)
% --cycle;

\path [draw=sdeBlackBox, fill=sdeBlackBox, opacity=0.6, line width=0pt]
(axis cs:0,-0.150000005960464)
--(axis cs:0,-0.150000005960464)
--(axis cs:0.150000005960464,-0.16198343038559)
--(axis cs:0.300000011920929,-0.162549749016762)
--(axis cs:0.449999958276749,-0.157338619232178)
--(axis cs:0.600000023841858,-0.15493942797184)
--(axis cs:0.749999940395355,-0.14329420030117)
--(axis cs:0.899999916553497,-0.130920261144638)
--(axis cs:1.04999995231628,-0.124211609363556)
--(axis cs:1.20000004768372,-0.111247025430202)
--(axis cs:1.34999990463257,-0.0968700721859932)
--(axis cs:1.49999988079071,-0.0800301805138588)
--(axis cs:1.64999985694885,-0.0650585740804672)
--(axis cs:1.79999983310699,-0.0502677634358406)
--(axis cs:1.94999992847443,-0.0334164910018444)
--(axis cs:2.09999990463257,-0.0196623988449574)
--(axis cs:2.25,-0.0053260731510818)
--(axis cs:2.40000009536743,0.00613307999446988)
--(axis cs:2.54999995231628,0.0194452945142984)
--(axis cs:2.69999980926514,0.0261648949235678)
--(axis cs:2.84999990463257,0.0347142070531845)
--(axis cs:2.99999976158142,0.043149571865797)
--(axis cs:3.14999985694885,0.0468625873327255)
--(axis cs:3.29999971389771,0.0471566803753376)
--(axis cs:3.44999980926514,0.0481985509395599)
--(axis cs:3.59999966621399,0.0507206656038761)
--(axis cs:3.74999976158142,0.048932071775198)
--(axis cs:3.89999985694885,0.0470454022288322)
--(axis cs:4.05000019073486,0.0436205789446831)
--(axis cs:4.19999980926514,0.0399357825517654)
--(axis cs:4.34999990463257,0.0361162610352039)
--(axis cs:4.5,0.0303755160421133)
--(axis cs:4.65000009536743,0.0262506008148193)
--(axis cs:4.80000019073486,0.020082276314497)
--(axis cs:4.95000028610229,0.0156098827719688)
--(axis cs:5.09999990463257,0.00861900206655264)
--(axis cs:5.25,0.00348594831302762)
--(axis cs:5.39999961853027,-0.000926621607504785)
--(axis cs:5.55000019073486,-0.00544667104259133)
--(axis cs:5.69999980926514,-0.00886932387948036)
--(axis cs:5.84999990463257,-0.0126089174300432)
--(axis cs:5.99999952316284,-0.0160900931805372)
--(axis cs:6.15000009536743,-0.0189315397292376)
--(axis cs:6.29999971389771,-0.0200410336256027)
--(axis cs:6.44999980926514,-0.0228603109717369)
--(axis cs:6.59999942779541,-0.0209122803062201)
--(axis cs:6.75,-0.0233912840485573)
--(axis cs:6.89999961853027,-0.020913515239954)
--(axis cs:7.04999971389771,-0.0179597456008196)
--(axis cs:7.19999933242798,-0.0176254697144032)
--(axis cs:7.34999942779541,-0.0189189184457064)
--(axis cs:7.49999952316284,-0.0171254109591246)
--(axis cs:7.64999961853027,-0.015520304441452)
--(axis cs:7.79999971389771,-0.0160460919141769)
--(axis cs:7.94999980926514,-0.0161649789661169)
--(axis cs:7.94999980926514,-0.00851297844201326)
--(axis cs:7.94999980926514,-0.00851297844201326)
--(axis cs:7.79999971389771,-0.00775358080863953)
--(axis cs:7.64999961853027,-0.0114864185452461)
--(axis cs:7.49999952316284,-0.0128579270094633)
--(axis cs:7.34999942779541,-0.0129674766212702)
--(axis cs:7.19999933242798,-0.0134833622723818)
--(axis cs:7.04999971389771,-0.014221522025764)
--(axis cs:6.89999961853027,-0.0149406464770436)
--(axis cs:6.75,-0.0157131422311068)
--(axis cs:6.59999942779541,-0.0150149334222078)
--(axis cs:6.44999980926514,-0.0155411083251238)
--(axis cs:6.29999971389771,-0.0160574223846197)
--(axis cs:6.15000009536743,-0.0143646132200956)
--(axis cs:5.99999952316284,-0.0124998148530722)
--(axis cs:5.84999990463257,-0.00946487858891487)
--(axis cs:5.69999980926514,-0.00536013022065163)
--(axis cs:5.55000019073486,-0.000339988124324009)
--(axis cs:5.39999961853027,0.00237411353737116)
--(axis cs:5.25,0.00843487214297056)
--(axis cs:5.09999990463257,0.0130898468196392)
--(axis cs:4.95000028610229,0.0197646841406822)
--(axis cs:4.80000019073486,0.025815911591053)
--(axis cs:4.65000009536743,0.0318583995103836)
--(axis cs:4.5,0.0354444459080696)
--(axis cs:4.34999990463257,0.0376520045101643)
--(axis cs:4.19999980926514,0.0429675504565239)
--(axis cs:4.05000019073486,0.0478677861392498)
--(axis cs:3.89999985694885,0.0502549484372139)
--(axis cs:3.74999976158142,0.0545921288430691)
--(axis cs:3.59999966621399,0.0546524561941624)
--(axis cs:3.44999980926514,0.0577223710715771)
--(axis cs:3.29999971389771,0.0578179880976677)
--(axis cs:3.14999985694885,0.0562910586595535)
--(axis cs:2.99999976158142,0.0489788204431534)
--(axis cs:2.84999990463257,0.0434478744864464)
--(axis cs:2.69999980926514,0.0341553390026093)
--(axis cs:2.54999995231628,0.0238985046744347)
--(axis cs:2.40000009536743,0.0127103850245476)
--(axis cs:2.25,0.000949563342146575)
--(axis cs:2.09999990463257,-0.0131893362849951)
--(axis cs:1.94999992847443,-0.029981330037117)
--(axis cs:1.79999983310699,-0.0460139587521553)
--(axis cs:1.64999985694885,-0.0636057257652283)
--(axis cs:1.49999988079071,-0.0738615542650223)
--(axis cs:1.34999990463257,-0.0866949781775475)
--(axis cs:1.20000004768372,-0.10085517168045)
--(axis cs:1.04999995231628,-0.114395529031754)
--(axis cs:0.899999916553497,-0.127375289797783)
--(axis cs:0.749999940395355,-0.137850105762482)
--(axis cs:0.600000023841858,-0.145033180713654)
--(axis cs:0.449999958276749,-0.150222778320312)
--(axis cs:0.300000011920929,-0.158768072724342)
--(axis cs:0.150000005960464,-0.15725927054882)
--(axis cs:0,-0.150000005960464)
--cycle;

\end{axis}

==> figures/mass_spring_damper/spring_mass_illustration.tex <==
\begin{tikzpicture}[black!75,thick]
 
\newlength{\wallOffset}
\newlength{\wallWidth}
\newlength{\wallHeight}
\newlength{\wallCompositeHeight}
\newlength{\springOneWidth}
\newlength{\springTwoWidth}
\newlength{\massHeight}
\newlength{\massWidth}
\newlength{\damperHeight}
\newlength{\damperWidth}
\newlength{\groundWidth}
\newlength{\groundHeight}
\newlength{\springDampSep}
\newlength{\forceVecLength}

\setlength{\wallOffset}{-3cm}
\setlength{\wallWidth}{0.2cm}
\setlength{\wallHeight}{0.75cm}
\setlength{\wallCompositeHeight}{1.5cm}
\setlength{\springOneWidth}{2cm}
\setlength{\springTwoWidth}{1.6cm}
\setlength{\massHeight}{0.75cm}
\setlength{\massWidth}{1cm}
\setlength{\damperHeight}{0.1cm}
\setlength{\damperWidth}{0.2cm}
\setlength{\groundWidth}{3.5cm}
\setlength{\groundHeight}{0.2cm}
\setlength{\springDampSep}{0.3cm}
\setlength{\forceVecLength}{0.5cm}

% \tikzstyle{spring}=[thick,decorate,decoration={zigzag,pre length=0.3cm,post
% length=0.3cm,segment length=6}]
\tikzstyle{spring}=[
    decorate,
    decoration={
        coil,
        aspect=0.3, 
        segment length=1.2mm, 
        amplitude=1mm, 
        pre length=3mm,
        post length=3mm,
    }
]

\tikzstyle{damper}=[
    decorate,
    thick,
    decoration={
        markings,  
        mark connection node=dmp,
        mark=at position 0.5 with {
            \node (dmp) [
                thick,
                inner sep=0pt,
                transform shape,
                rotate=-90,
                minimum width=\damperWidth,
                minimum height=\damperHeight,
                draw=none
            ] {};a
            \draw [thick] ($(dmp.north east)+(2pt,0)$) -- (dmp.south east) -- (dmp.south west) -- ($(dmp.north west)+(2pt,0)$);
            \draw [thick] ($(dmp.north)+(0,-3pt)$) -- ($(dmp.north)+(0,3pt)$);
        }
    }, 
]

%% Draw subsystem 1
% Wall 1
\node [
    pattern = north east lines,
    minimum width=\wallWidth,
    minimum height=\wallHeight,
] (wall1) {};
\draw[thick] ($(wall1.east) + (0, -\wallHeight / 2)$) -- ($(wall1.east) + (0,\wallHeight / 2)$);

% Ground 1
\node[
    pattern = north east lines,
    minimum width=\groundWidth,
    minimum height=\groundHeight,
    below right = \wallHeight/2 and 0.0cm of wall1.west,
] (ground1) {};
\draw[thick] ($(wall1.east) + (0, -\wallHeight / 2)$) -- ($(ground1.east) + (0.0, \groundHeight / 2)$);

% \fill [pattern = north east lines] (\wallOffset, - \wallHeight / 2) rectangle ++(\wallWidth, \wallHeight);
% \draw[thick] (\wallOffset + \wallWidth, - \wallHeight / 2) -- ++(0.0cm, \wallHeight);
 
% Mass 1
\node[draw,
    color=submodel1Color,
    fill=submodel1Color,
    minimum width=1cm,
    minimum height=0.75cm,
    anchor=west,
    right = \springOneWidth of wall1,
    text=white] (M1) {$m_{1}$};
 
% Spring 1
\draw[spring, color=submodel1Color] ($(wall1.east) + (0.0, \springDampSep / 2)$) -- ($(M1.west) + (0.0, \springDampSep / 2)$); % node[midway, above=0.25cm,black]{$k_{1}$}; 

% Damper 1
\draw[damper, color=submodel1Color] ($(wall1.east) + (0.0, -\springDampSep / 2)$) -- ($(M1.west) + (0.0, -\springDampSep / 2)$); % node[midway, below=0.2cm, black]{$b_{1}$};
 
% Label
% \node[above=0.65cm of ground1.north, color=submodel1Color] (subsystem1Label) {Subsystem 1};
 
\end{tikzpicture}

==> rebuttal/rebuttal_cartpole_rl_performance_bar_chart.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
width=1.0*\columnwidth, 
height=5.0cm,
tick align=inside,
tick pos=left,
x grid style={darkgray176},
xmin=-0.117, xmax=1.577,
xtick style={draw=none},
xticklabel style={rotate=0, font=\scriptsize},
y grid style={darkgray176},
ymin=0, ymax=644.612958758698,
ytick style={color=black},
axis y line*=left,
axis x line* = bottom,
align={center},
ylabel={\footnotesize Episodic Reward},
yticklabel style={font=\footnotesize},
xtick={0, 0.21, 0.38, 0.54, 0.78, 0.96, 1.12, 1.28, 1.45},
xticklabels={
    \shortstack[c]{Ground Truth \\ Dynamics}, 
    \shortstack[c]{Neural SDE\\(Ours)},
    \shortstack[c]{Neural ODE},
    \shortstack[c]{Prob. \\ Ensemble},
    \shortstack[c]{Neural SDE \\ w/ Side Info.\\(Ours)},
    \shortstack[c]{Neural ODE \\ w/ Side Info.},
    \shortstack[c]{Neural SDE\\(Ours)},
    \shortstack[c]{Neural ODE},
    \shortstack[c]{Prob. \\ Ensemble},
    },
ytick={0, 89, 303, 513},
yticklabels={0, 89, 303, 513},
]
\draw[draw=black, pattern=crosshatch, pattern color=groundTruth] (axis cs:-0.04,0) rectangle (axis cs:0.04,512.787435934102);

\draw[draw=black, pattern=crosshatch, pattern color=sdeBlackBox] (axis cs:0.16,0) rectangle (axis cs:0.24,508.451471328089);
\draw[draw=none, draw=black, pattern=grid, pattern color=sdeBlackBox] (axis cs:0.24,0) rectangle (axis cs:0.28,532.09796382886);

\draw[draw=black,pattern=crosshatch, pattern color=neuralODE] (axis cs:0.32,0) rectangle (axis cs:0.4,471.086210294116);
\draw[draw=none, draw=black, pattern=grid, pattern color=neuralODE] (axis cs:0.4,0) rectangle (axis cs:0.44,500.078508200427);

\draw[draw=black,pattern=crosshatch, pattern color=gaussianEnsemble] (axis cs:0.48,0) rectangle (axis cs:0.56,303.249820859697);
\draw[draw=black,pattern=grid, pattern color=gaussianEnsemble] (axis cs:0.56,0) rectangle (axis cs:0.6,320.534961018009);

\draw[draw=black,pattern=crosshatch, pattern color=sdeSideInfo] (axis cs:0.74,0) rectangle (axis cs:0.82,502.682927880094);
\draw[draw=black,pattern=grid, pattern color=sdeSideInfo] (axis cs:0.82,0) rectangle (axis cs:0.86,534.835072410437);

\draw[draw=black,pattern=crosshatch, pattern color=neuralODESideInfo] (axis cs:0.9,0) rectangle (axis cs:0.98,447.226336444784);
\draw[draw=black,pattern=grid, pattern color=neuralODESideInfo] (axis cs:0.98,0) rectangle (axis cs:1.02,544.765759529528);

\draw[draw=black,pattern=crosshatch, pattern color=sdeBlackBox] (axis cs:1.06,0) rectangle (axis cs:1.14,447.478373237097);
\draw[draw=black,pattern=grid, pattern color=sdeBlackBox] (axis cs:1.14,0) rectangle (axis cs:1.18,519.798828469653);

\draw[draw=black,pattern=crosshatch, pattern color=neuralODE] (axis cs:1.22,0) rectangle (axis cs:1.3,374.441862628853);
\draw[draw=black,pattern=grid, pattern color=neuralODE] (axis cs:1.3,0) rectangle (axis cs:1.34,478.656912532898);

\draw[draw=black,pattern=crosshatch, pattern color=gaussianEnsemble] (axis cs:1.38,0) rectangle (axis cs:1.46,88.5613818263148);
\draw[draw=black,pattern=grid, pattern color=gaussianEnsemble] (axis cs:1.46,0) rectangle (axis cs:1.5,581.01651229493);

\path [draw=black, semithick]
(axis cs:0,482.62239139825)
--(axis cs:0,542.952480469953);
\path [draw=black, semithick]
(axis cs:0.2,472.570529451489)
--(axis cs:0.2,544.332413204689);
\path [draw=black, semithick]
(axis cs:0.26,503.250778625692)
--(axis cs:0.26,560.945149032029);
\path [draw=black, semithick]
(axis cs:0.36,417.443837760582)
--(axis cs:0.36,524.728582827651);
\path [draw=black, semithick]
(axis cs:0.42,477.126401260527)
--(axis cs:0.42,523.030615140327);
\path [draw=black, semithick]
(axis cs:0.52,246.362454405873)
--(axis cs:0.52,360.137187313522);
\path [draw=black, semithick]
(axis cs:0.58,244.098147283769)
--(axis cs:0.58,396.971774752249);
\path [draw=black, semithick]
(axis cs:0.78,442.180654118115)
--(axis cs:0.78,563.185201642073);
\path [draw=black, semithick]
(axis cs:0.84,504.652816036883)
--(axis cs:0.84,565.01732878399);
\path [draw=black, semithick]
(axis cs:0.94,363.463310226243)
--(axis cs:0.94,530.989362663325);
\path [draw=black, semithick]
(axis cs:1,518.167698205653)
--(axis cs:1,571.363820853403);
\path [draw=black, semithick]
(axis cs:1.1,382.539134250776)
--(axis cs:1.1,512.417612223417);
\path [draw=black, semithick]
(axis cs:1.16,480.968231321273)
--(axis cs:1.16,558.629425618033);
\path [draw=black, semithick]
(axis cs:1.26,311.30540613741)
--(axis cs:1.26,437.578319120296);
\path [draw=black, semithick]
(axis cs:1.32,436.587826123178)
--(axis cs:1.32,520.725998942618);
\path [draw=black, semithick]
(axis cs:1.42,2.40959749059252)
--(axis cs:1.42,174.713166162037);
\path [draw=black, semithick]
(axis cs:1.48,548.115921010147)
--(axis cs:1.48,613.917103579712);

\addplot [semithick, black, mark=-, mark size=2, mark options={solid}, only marks]
table {%
0 482.62239139825
0.2 472.570529451489
0.26 503.250778625692
0.36 417.443837760582
0.42 477.126401260527
0.52 246.362454405873
0.58 244.098147283769
0.78 442.180654118115
0.84 504.652816036883
0.94 363.463310226243
1 518.167698205653
1.1 382.539134250776
1.16 480.968231321273
1.26 311.30540613741
1.32 436.587826123178
1.42 2.40959749059252
1.48 548.115921010147
};

\addplot [semithick, black, mark=-, mark size=2, mark options={solid}, only marks]
table {%
0 542.952480469953
0.2 544.332413204689
0.26 560.945149032029
0.36 524.728582827651
0.42 523.030615140327
0.52 360.137187313522
0.58 396.971774752249
0.78 563.185201642073
0.84 565.01732878399
0.94 530.989362663325
1 571.363820853403
1.1 512.417612223417
1.16 558.629425618033
1.26 437.578319120296
1.32 520.725998942618
1.42 174.713166162037
1.48 613.917103579712
};
\end{axis}

\draw [decorate, decoration = {calligraphic brace, mirror}, very thick] (6.1cm, 3.4cm) --  (2.1cm, 3.4cm);
\node(labelForRandomDataset) [font=\scriptsize, align=left] at (4.1cm, 3.7cm) {\shortstack[c]{\textit{random dataset}}};

\draw [decorate, decoration = {calligraphic brace, mirror}, very thick] (13.5cm, 3.4cm) --  (6.9cm, 3.4cm);
\node(labelForLearnedDataset) [font=\scriptsize, align=left] at (10.2cm, 3.7cm) {\shortstack[c]{\textit{on-policy dataset}}};

% \draw [gray, decorate, decoration = {calligraphic brace}, thick] (8.2cm, -0.1cm) --  (8.2cm, -0.9cm);
% \node(labelForLabels) [font=\scriptsize, align=left] at (9.2cm, -0.5cm) {\shortstack[l]{Model used to \\ train policy}};

\begin{customlegend}[
    legend columns=2, 
    legend style={
        align=left, 
        column sep=1.0ex, 
        font=\scriptsize, 
        % draw=white!50!black,
        draw=none,
        fill=white,
        fill opacity=0.8,
        rounded corners=1mm,
        at={(120.0mm, -10.0mm)},
    }, 
    legend entries={\shortstack[l]{Policy evaluated using true dynamics}, \shortstack[l]{Policy evaluated using learned dynamics}}
]
    \addlegendimage{area legend,pattern=crosshatch, pattern color=black}
    \addlegendimage{area legend,pattern=grid, pattern color=black}
\end{customlegend}

\end{tikzpicture}

